EMR-MSF: Self-Supervised Recurrent Monocular Scene Flow Exploiting Ego-Motion Rigidity

Self-supervised monocular scene flow estimation, aiming to understand both 3D structures and 3D motions from two temporally consecutive monocular images, has received increasing attention for its simple and economical sensor setup. However, the accuracy of current methods suffers from the bottleneck of less-efficient network architecture and lack of motion rigidity for regularization. In this paper, we propose a superior model named EMR-MSF by borrowing the advantages of network architecture design under the scope of supervised learning. We further impose explicit and robust geometric constraints with an elaborately constructed ego-motion aggregation module where a rigidity soft mask is proposed to filter out dynamic regions for stable ego-motion estimation using static regions. Moreover, we propose a motion consistency loss along with a mask regularization loss to fully exploit static regions. Several efficient training strategies are integrated including a gradient detachment technique and an enhanced view synthesis process for better performance. Our proposed method outperforms the previous self-supervised works by a large margin and catches up to the performance of supervised methods. On the KITTI scene flow benchmark, our approach improves the SF-all metric of the state-of-the-art self-supervised monocular method by 44% and demonstrates superior performance across sub-tasks including depth and visual odometry, amongst other self-supervised single-task or multi-task methods.

==> bak_tables_and_figures.tex <==
\begin{table}[h]
\centering
\resizebox{0.75\linewidth}{!}{
\begin{tabular}{l|cc|c}
\toprule[2pt]
\multirow{2}{*}{Method} & \multicolumn{2}{c|}{Train}       & Test             \\ \cline{2-4} 
                                                 & EPE           & F1-all           & F1-all           \\ \hline
GeoNet \cite{yin2018geonet}                                           & 10.81         & -                & -                \\
DF-Net \cite{zou2018df}                                           & 8.98          & 26.01          & 25.70          \\
Self-Mono-SF \cite{hur2020self}                                     & 7.51          & 23.49          & 23.54          \\
CC-uft \cite{ranjan2019competitive}                                           & 5.66          & 20.93          & 25.27          \\
UnOS \cite{wang2019unos}                                             & 5.58          & -                & 18.00          \\
EPC++ \cite{luo2019every}                                            & 5.43          & 19.64          & 20.52          \\
UnRigidFlow \cite{liu2019unsupervised}              & 5.19          & 14.68          & \textbf{11.66} \\
EffiScene \cite{jiao2021effiscene}              & 4.20          & 14.31          & 13.08          \\
\textbf{Ours}                         & \textbf{3.46} & \textbf{11.58} & 11.93          \\
\bottomrule[2px]
\end{tabular}
}
\caption{Comparison of optical flow estimation on KITTI 2015 Training Set.}
\label{tab3_optical_train}
\end{table}


\begin{figure}[t]
    \centering
    \begin{tabular}{c}
        \includegraphics[width=0.95\linewidth]{figs/fig_raft_3d_crop.pdf}
    \end{tabular}
    \caption{Comparison with RAFT-3D pretrained on Flyingthings.}
    \label{fig_ablation}
\end{figure}


\begin{table*}[h]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{l|c|cccc|ccc}
\toprule[2pt]
Method       & Sup.                      & Abs Rel $\downarrow$       & Sq Rel $\downarrow$        & RMSE $\downarrow$          & RMSE log $\downarrow$      & A1 $\uparrow$            & A2 $\uparrow$            & A3 $\uparrow$            \\ \hline
Monodepth2   \cite{godard2019digging}       & M             & 0.115          & 0.903          & 4.863          & 0.193          & 0.877          & 0.959          & 0.981          \\
PackNet-SfM  \cite{guizilini20203d}         & M             & 0.111          & 0.785          & 4.601          & 0.189          & 0.878          & 0.960          & 0.982          \\
DIFFNet      \cite{zhou_diffnet}            & M             & 0.102          & 0.764          & 4.483          & 0.180          & 0.896          & 0.965          & 0.983          \\
RA-Depth     \cite{he2022ra}                & M             & \textbf{0.096} & \textbf{0.632} & \textbf{4.216} & \textbf{0.171} & \textbf{0.903} & \textbf{0.968} & \textbf{0.985} \\ \hline
Monodepth2   \cite{godard2019digging}       & S             & 0.109          & 0.873          & 4.960          & 0.209          & 0.864          & 0.948          & 0.975          \\
FAL-Net      \cite{gonzalezbello2020forget} & S            & 0.097          & 0.590          & 3.991          & 0.177          & 0.893          & 0.966          & 0.984          \\
PLADE-Net    \cite{gonzalez2021plade}       & S            & 0.092          & 0.626          & 4.046          & 0.175          & 0.896          & 0.965          & 0.984          \\
% SDFA-Net (w/o RC)    \cite{zhou2022self}            & S             & 0.093          & 0.594          & 4.167          & 0.179          & 0.892          & 0.964          & 0.983          \\
SDFA-Net     \cite{zhou2022self}            & S            & \textbf{0.090} & \textbf{0.538} & \textbf{3.896} & \textbf{0.169} & \textbf{0.906} & \textbf{0.969} & \textbf{0.985} \\ \hline
EPC++        \cite{luo2019every}            & MS            & 0.127          & 0.936          & 5.008          & 0.209          & 0.841          & 0.946          & 0.979          \\
Self-Mono-SF \cite{hur2020self}             & MS            & 0.125          & 0.978          & 4.877          & 0.208          & 0.851          & 0.950          & 0.978          \\
Monodepth2   \cite{godard2019digging}       & MS            & 0.106          & 0.818          & 4.750          & 0.196          & 0.874          & 0.957          & 0.979          \\
DIFFNet      \cite{zhou_diffnet}            & MS            & 0.101          & 0.749          & 4.445          & 0.179          & 0.898          & 0.965          & 0.983          \\
RAFT-MSF     \cite{bayramli2022raft}        & MS            & 0.093          & 0.781          & 4.321          & 0.186          & \textbf{0.901} & 0.960          & 0.981          \\
\textbf{Ours}                               & MS            & \textbf{0.088} & \textbf{0.572} & \textbf{4.146} & \textbf{0.174} & 0.899          & \textbf{0.966} & \textbf{0.984} \\
\bottomrule[2pt]
\end{tabular}
}
\caption{Comparison of depth estimation on KITTI Eigen Test Set.}
\label{tab4_depth_eigen}
\end{table*}

